A Projectional Ansatz to Reconstruction

Recently the field of inverse problems has seen a growing usage of mathematically only partially understood learned and non-learned priors. Based on first principles, we develop a projectional approach to inverse problems that addresses the incorporation of these priors, while still guaranteeing data consistency. We implement this projectional method (PM) on the one hand via very general Plug-and-Play priors and on the other hand, via an end-to-end training approach. To this end, we introduce a novel alternating neural architecture, allowing for the incorporation of highly customized priors from data in a principled manner. We also show how the recent success of Regularization by Denoising (RED) can, at least to some extent, be explained as an approximation of the PM. Furthermore, we demonstrate how the idea can be applied to stop the degradation of Deep Image Prior (DIP) reconstructions over time.

==> dip_old.tex <==
In this section we discuss how one can implement the central idea of finding an element in $U\cap V$ for the case where $U$ is given by all possible reconstructions from a Deep Image Prior (DIP).

The idea of using DIP to solve inverse problems, as described by \citet{van2018compressed}, is to minimize the functional
\begin{equation}
    L_\text{DIP}(\Theta) := \frac{1}{2}\|AG_\Theta(z) - y^\delta\|^2
\end{equation}
with regard to $\Theta$, where $G_\Theta(z)$ is an untrained neural network with a fixed random input $z$ and parameters $\Theta$. The reconsturction is then given via $G_\Theta(z)$, i.e.\ the output of the network.

We present two ways in which one can modify the DIP functional to find a valid and plausible reconstruction. The first possible functional is
\begin{equation}
    L_\text{DIP+PM}(\Theta) := \frac{1}{2}\|G_\Theta(z) - P_{V(A, y^\delta, \delta)}G_\Theta(z)\|^2.
\end{equation}
Here the reconstruction would be given by $P_{V(A, y^\delta, \delta)}G_\Theta(z)$ or $G_\Theta(z)$ after the minimization process. Since the choice $P_{V(A, y^\delta, \delta)}G_\Theta(z)$ guarantees that the reconstruction is valid without relying on the fact that the highly non-convex minimization does not get stuck in a local minimum, we use it as our reconstruction when using this functional.

The second possible functional we propose is
\begin{equation}
    L_\text{DIP+$\delta$}(\Theta) := \left(\|AG_\Theta(z) - y^\delta\|^2 - \delta^2\right)^2.
\end{equation}
Here the reconstruction is given by $G_\Theta(z)$ after the minimization.

On the one hand the functional $L_\text{DIP+$\delta$}$, can not guarantee that the in practice reached reconstruction is valid (due to the non-convexity of $G_\cdot(z)$), but on the other hand this functional does not rely on $P_V$, which makes a single iteration much faster to compute.

We now compare these three different approaches in the same setup as used in Section~\ref{sec:red} for RED and the PM based on BM3D. As the DIP network we use the ``skip net'' UNet described in the original DIP paper (\citet{ulyanov2018deep}) and Adam with standard settings, which we found to work best for our DIP reconstructions. The results can be found in Figure~\ref{fig:dip_results}. Like in Section~\ref{sec:red} we compare the PSNR, SSIM and $\frac{\|y - y'\|}{\|y\|}$, where $y=Ax$ is the noise free measurement of the ground truth and $y'=Ax^\dagger$ the noise free measurement of the reconstruction. We plot the reconstruction over time, not over the number of iterations, because one iteration of $L_\text{DIP+PM}$ takes approximately $10$ times longer than one of $L_\text{DIP}$ or $L_\text{DIP+$\delta$}$, which both take approximately the same time per step. We stopped the optimization (ran in parallel on an Nvidia GeForce GTX 1080 ti) after TODO hours. Samples of the actual reconstructions can be found in Figure~\ref{fig:dip_reconstructions_1e-2},~\ref{fig:dip_reconstructions_1e-1} and~\ref{fig:dip_reconstructions_3e-1} in the appendix. DIP reached TODO iterations DIP+PM reached TODO iterations and DIP+$\delta$ reached TODO iterations. We find that both modified functional show, accept for short spikes, much less deterioration of the reconstruction overtime and it outperforms the vanilla DIP especially for higher levels of noise.

\begin{figure}
    \centering
    \begin{minipage}{.319\textwidth}
    \includegraphics[width=1\linewidth]{figures/reconstructions/dip/dip_01.png}
    \subcaption{1\% noise}
    \end{minipage}
    \begin{minipage}{.319\textwidth}
    \includegraphics[width=1\linewidth]{figures/reconstructions/dip/dip_10.png}
    \subcaption{10\% noise}
    \end{minipage}
    \begin{minipage}{.319\textwidth}
    \includegraphics[width=1\linewidth]{figures/reconstructions/dip/dip_30.png}
    \subcaption{30\% noise}
    \end{minipage}
    \caption{The behavior of the minimization of $L_\text{DIP}$ (red) and of $L_\text{DIP+$\delta$}$ (cyan) over the course of the reconstruction.}
    \label{fig:dip_results}
\end{figure}

==> numerical_results.tex <==
\begin{itemize}
    \item Show STL10 and LIDC results. for:
        \begin{itemize}
            \item TV
            \item RED
            \item DIP
            \item BM3D
            \item vNPA
            \item FBP
        \end{itemize}
    \item Show MNIST results?
    \item describe setup (last step!)
    \item Analyse $\rightarrow$ Concentration of Measure?
\end{itemize}

\input{figures/reconstructions/reconstructions_cs_big_0/figure.tex}
\input{figures/reconstructions/reconstructions_cs_big_1/figure.tex}
\input{figures/reconstructions/reconstructions_cs_slim_0/figure.tex}
\input{figures/reconstructions/reconstructions_cs_slim_1/figure.tex}
\input{figures/reconstructions/reconstructions_radon_slim_0/figure.tex}
\input{figures/reconstructions/reconstructions_radon_slim_1/figure.tex}
\input{figures/reconstructions/reconstructions_radon_big_0/figure.tex}
\input{figures/reconstructions/reconstructions_radon_big_1/figure.tex}
